Generating bilingual example sentences with large language models as lexicography assistants

We present a study of LLMs' performance in generating and rating example sentences for bilingual dictionaries across languages with varying resource levels: French (high-resource), Indonesian (mid-resource), and Tetun (low-resource), with English as the target language. We evaluate the quality of LLM-generated examples against the GDEX (Good Dictionary EXample) criteria: typicality, informativeness, and intelligibility. Our findings reveal that while LLMs can generate reasonably good dictionary examples, their performance degrades significantly for lower-resourced languages. We also observe high variability in human preferences for example quality, reflected in low inter-annotator agreement rates. To address this, we demonstrate that in-context learning can successfully align LLMs with individual annotator preferences. Additionally, we explore the use of pre-trained language models for automated rating of examples, finding that sentence perplexity serves as a good proxy for typicality and intelligibility in higher-resourced languages. Our study also contributes a novel dataset of 600 ratings for LLM-generated sentence pairs, and provides insights into the potential of LLMs in reducing the cost of lexicographic work, particularly for low-resource languages.

==> process_generate_examples.tex <==

\usetikzlibrary{shapes.geometric, arrows.meta, positioning}

\tikzset{
    base/.style = {draw, text width=2.5cm, align=center, minimum height=1em, font=\small},
    inout/.style = {base, rectangle, rounded corners},
    process/.style = {base, rectangle, fill=blue!30},
    gate/.style = {base, chamfered rectangle, fill=red!30},
}


\begin{tikzpicture}[node distance=1.2cm and 0.5cm, auto]
    \node [process] (50src) {Sample of 50 source words in top 10k for lang};
    \node [inout, right=1.5cm of 50src] (translate) {50 word pairs};
    \node [inout, right=1.5cm of translate] (sents) {50 word \& sentence pairs};
    \node [inout, right=1.5cm of translate] (sents) {50 pairs with annotations against GDEX};
    \node 50 source words at random 
    % % Nodes
    % \node [process] (get10k) {Get top 10k words for source lang};
    % \node [inout, right=1.5cm of get10k] (select50) {Sample 50 words};
    % \node [inout, right=1.5cm of select50] (translate) {Translate to English};
    % \node [inout, right=1.5cm of translate] (llmgenerate) {Generate 50 sentence pairs};
    % \node [inout, right=1.5cm of llmgenerate] (rate) {Rate against GDEX criteria};

    % % Arrows
    % \draw[-Latex] (get10k) -- (select50);
    % \draw[-Latex] (select50) -- (translate);
    % \draw[-Latex] (translate) -- (llmgenerate);
    % \draw[-Latex] (llmgenerate) -- (rate);
\end{tikzpicture}

